Image is All You Need to Empower Large-scale Diffusion Models for In-Domain Generation

In-domain generation aims to perform a variety of tasks within a specific domain, such as unconditional generation, text-to-image, image editing, 3D generation, and more. Early research typically required training specialized generators for each unique task and domain, often relying on fully-labeled data. Motivated by the powerful generative capabilities and broad applications of diffusion models, we are driven to explore leveraging label-free data to empower these models for in-domain generation. Fine-tuning a pre-trained generative model on domain data is an intuitive but challenging way and often requires complex manual hyper-parameter adjustments since the limited diversity of the training data can easily disrupt the model's original generative capabilities. To address this challenge, we propose a guidance-decoupled prior preservation mechanism to achieve high generative quality and controllability by image-only data, inspired by preserving the pre-trained model from a denoising guidance perspective. We decouple domain-related guidance from the conditional guidance used in classifier-free guidance mechanisms to preserve open-world control guidance and unconditional guidance from the pre-trained model. We further propose an efficient domain knowledge learning technique to train an additional text-free UNet copy to predict domain guidance. Besides, we theoretically illustrate a multi-guidance in-domain generation pipeline for a variety of generative tasks, leveraging multiple guidances from distinct diffusion models and conditions. Extensive experiments demonstrate the superiority of our method in domain-specific synthesis and its compatibility with various diffusion-based control methods and applications.

==> sec/0_abstract.tex <==
\begin{abstract}
Despite the impressive capabilities of large-scale text-to-image diffusion models in open-world image generation, they still meet challenges in synthesizing high-fidelity images in specific domains (e.g., human faces), especially when compared to specialized unconditional generators.
In this paper, we investigate the potential of leveraging a pre-trained diffusion model to achieve controllable and photorealistic domain-specific generation by learning from image-only data. It indicates that we can build a poweful domain generator
Although directly fine-tuning seems like an intuitive approach, we point out that it often leads to issues including the tradeoff between fidelity and controllability, as well as unconditional guidance drift.
To address these challenges, we propose a simple yet effective guidance-decoupled framework for both training and inference. This framework introduces the idea of multi-guidance generation, decoupling a domain-specific guidance (named domain guidance) from the conditional guidance used in classifier-free guidance mechanisms.
We further introduce a text-free UNet copy that learns domain guidance from image data, which then guides the denoising process by maximizing the likelihood of domain probability during inference.
Additionally, to improve the efficiency of controllable generation, we propose an adaptive time-aware guidance scheduling mechanism, which dynamically adjusts the presence of each guidance during generation, reducing extra computational costs.
Our proposed framework efficiently combines domain knowledge from image-only datasets with the controllability of diffusion priors. 
Extensive experiments demonstrate the superiority of our method in domain-specific synthesis and its compatibility with various diffusion-based control methods and applications.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure*}[t!]
	\begin{center}
		\includegraphics[width=1.0\linewidth]{figure/sample.pdf}
	\end{center}
	\vspace{-3mm}
	\caption{\textbf{Concept personalization.} In this work, we introduce a novel diffusion-based task, termed concept personalization, where diffusion priors are customized to achieve faithful, diverse, and controllable generation of a given concept, using image-only data. It is also training-free to integrate with off-the-shelf controlling methods (\eg ControlNet and style LoRA).}
	\vspace{-4mm}
	\label{fig:introduce}
\end{figure*}

Thanks to billion-scale image-text datasets~\cite{caesar2018coco,schuhmann2021laion,ramesh2022hierarchical,schuhmann2022laion} and the development of large-scale natural language models~\cite{devlin2018bert,raffel2020exploring,radford2021learning}, the research on diffusion models in recent years has expanded the boundaries of artificial intelligence generated content, significantly enhancing the diversity and controllability of the generated content \cite{rombach2022high}. 

As illustrated in Fig~\ref{fig:introduce}(a), while existing text-to-image models are capable of generating \texttt{a photo of porcelain}, the results fail to meet human preferences. This observation prompts a novel idea: can we instruct the generator on the desired appearance of the concept? 
In this work, we introduce the task of concept personalization, which aims to generate faithful and human-preferred concept images with powerful control capability. This task is required to inherit the diverse control capabilities of diffusion priors, encompassing not only text-guided generation but also compatibility with existing controllable generation methods. This integration facilitates more versatile concept generation applications, such as stylized generation or image-to-image translation, as shown in Fig~\ref{fig:introduce}(b).
Moreover, to broaden the scope of this task and enhance its practicality, we propose implementing it solely with image data, thus eliminating the need for costly annotations. 
%For example, by utilizing a customized porcelain image dataset, the generator should be capable of producing photorealistic porcelain photos in response to text prompts.

%Moreover, thanks to the development of diffusion-based downstream works, this task enables a wide range of generative applications. without the need for application-specific data and extra training, such as stylized generation and image-to-image translation. It can integrate seamlessly with these off-the-shelf controllable generation methods to realize more comprehensive applications, as depicted in the right part of Fig~\ref{fig:introduce}. 
%Notably, these plugins require no additional training for concept generation, allowing for straightforward implementation with ControlNet trained on Stable Diffusion v1.5 alongside our concept generator.

Despite fine-tuning diffusion models~\cite{gal2022image,ruiz2023DreamBooth,qiu2023controlling} with prompt templates (\eg \texttt{a photo of a <placeholder>}) or caption models\cite{alayrac2022flamingo,li2023blip,liu2024visual} being an intuitive solution to this task, it would severely degrade generative quality. First, it gains a worse performance of fidelity-controllability tradeoff during personalization, since training on concept images with broad visual distributions without accurate text labels breaks the visual-language relation in diffusion priors. 
In addition, we identify an overlooked issue: training in a narrow domain leads to the generation of artifacts in the output. Meanwhile, even with adequate training, the model still struggles to produce high-quality concept images.

In this work, we first identify these two issues are caused by conditional guidance and unconditional guidance catastrophic forgetting during personalization, respectively. These two guidances are integrated by classifier-free guidance for improved generative capability, which is employed in most text-to-image diffusion models.
Hence, we propose a guidance-decoupled personalization framework to address these challenges.
We decouple the conditional guidance in CFG into two parts: concept guidance, which is optimized in personalization to enhance fidelity, and control guidance, which is preserved for controllability. 
With introducing multiple guidances in the synthesis process, the control guidance and unconditional guidance, which we want to preserve during personalization, are directly predicted by diffusion priors, while the concept guidance is predicted by an independent diffusion model.
Additionally, we construct a null-text Concept-centric Diffusion Model to learn concept information in a concise way. We also develop efficient training techniques in concept personalization to accelerate its convergence. 

% 5. Experiments
We conduct extensive experiments to demonstrate the effects of our proposed task and validate the superiority of our approach. 
To summarize, our contributions are as follows:
\begin{itemize}
\item[$\bullet$] We introduce the text-free concept personalization task, aiming to align concept generation with given images and generate concept images with high fidelity and controllability.
\item[$\bullet$] We identify two challenges of fidelity-controllability tradeoff and unconditional guidance drift in this task and reveal their root causes: conditional guidance and unconditional guidance catastrophic forgetting in personalization.
\item[$\bullet$] We propose a guidance-decoupled personalization framework to address this task, which decouples concept guidance to learn concept information with other guidance preserved. Besides, we design a null-text concept diffusion model to estimate concept guidance and develop efficient personalization techniques.
\item[$\bullet$] We conduct extensive experiments across several concepts to illustrate the effects of our proposed task and method. Through concept personalization, a variety of controllable generation tasks can be achieved by using only image data.
\end{itemize}


==> sec/2_related_works.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
